NoiseBench: Benchmarking the Impact of Real Label Noise on Named Entity Recognition

Available training data for named entity recognition (NER) often contains a significant percentage of incorrect labels for entity types and entity boundaries. Such label noise poses challenges for supervised learning and may significantly deteriorate model quality. To address this, prior work proposed various noise-robust learning approaches capable of learning from data with partially incorrect labels. These approaches are typically evaluated using simulated noise where the labels in a clean dataset are automatically corrupted. However, as we show in this paper, this leads to unrealistic noise that is far easier to handle than real noise caused by human error or semi-automatic annotation. To enable the study of the impact of various types of real noise, we introduce NoiseBench, an NER benchmark consisting of clean training data corrupted with 6 types of real noise, including expert errors, crowdsourcing errors, automatic annotation errors and LLM errors. We present an analysis that shows that real noise is significantly more challenging than simulated noise, and show that current state-of-the-art models for noise-robust learning fall far short of their theoretically achievable upper bound. We release NoiseBench to the research community.

==> additional_content/ablation_rt.tex <==

\section{Ablation: Sentiment Classification}

In addition to NER, which is the main focus of this paper, we also investigate how noise-robust approaches perform in the sentiment classification task when faced with real label noise. 

\subsection{Dataset} This task is represented by the Rotten Tomatoes Movie Reviews (\rottentomatoes) dataset \cite{pang-lee-2005-seeing}, which includes sentences extracted from online movie reviews aimed for binary classification based on whether the sentiment is positive or negative. We follow the methodology for the creation of \benchmark{} and create clean training and test splits, as well as 4 additional variants of the training set, labeled with different types of noise. The training set consists of 5000 examples from the \rottentomatoes~dataset, for which \citet{rodrigues2013learning} have published crowdsourced labels. Since the full \rottentomatoes~dataset contains 10000 examples, we include the remaining 5000 data points as our clean test set. We create 4 noisy variants of the training split: \noisecrowdbest, \noisecrowd, \noiseweak~and \noisellm \ in the same way as those in \benchmark{}. The resulting noise shares are shown in the first row in Table \ref{exp3_rt_results}. %, together with the summarized results of noise-robust methods are shown in Table 

% % , with their noise levels shown in Table \ref{conll_noise_shares_table}. For this task, we express the noise levels in terms of error rate, as a percentage ($100 - \%Accuracy$).

\subsection{Experimental setup}
We repeat the evaluation of noise-robust approaches on the sentiment classification task. As a baseline, we fine-tune an \texttt{xlm-roberta-large} transformer. % with the same parameters. 
In addition to the baseline, we again evaluate three noise-robust approaches, and provide the same theoretical upper bounds. 

\textbf{Noise-robust approaches.} Same as for NER, we evaluate Confident learning and Co-regularization for this task, however since BOND is a NER-specific approach, we evaluate another conceptually similar approach \textbf{COSINE} \citep{yu2021fine}. It is also a two-stage approach that follows a regular transformer fine-tuning objective in the first step (on weak labels), and a contrastive self-training objective to suppress label noise propagation afterwards. The self-training stage also relies on the high-confidence samples in order to update the model. Similarly to BOND, we stop the first stage manually after the 4th epoch, and limit the second stage to 6 epochs. We perform a small hyperparameter search in order to find the optimal ones for each noise type, as suggested by the authors.

\input{tables/rotten-tomatoes-sentiment/rt_results}

% The Rotten Tomatoes subset (the Sentiment benchmark) is split randomly, with 20\% of the sentences being included in the validation set.
% As a classification metric we calculate accuracy


\subsection{Results}

The results from this ablation experiment are presented in Table \ref{exp3_rt_results}.

\textbf{Noise share.} Regarding the noise shares of different types of noise, we can note that they are rather low in comparison to the corresponding \benchmark \ label sets, except for the Weak label set. This indicates that real label noise can have varying degrees of difficulty depending on the task.

\textbf{Noise robustness.}
 We can see that Co-regularization is a clear winner among the noise-robust learning approaches. Once again, the baseline is outperformed only slightly, but in this case, the theoretical upper bound is not that far away from the baseline, except for the Weak label set.

Furthermore, the \noiseclean~label set here actually probably corresponds to the \noiseexpert~label set of \benchmark, since there were no re-labeling efforts made when it comes to the Rotten Tomatoes dataset%, or any of the popular sentiment classification datasets for that matter
. This can explain why the \noisecrowdbest~upper bound is higher than the \noiseclean~baseline.

This ablation highlights the advantages of \benchmark, for evaluating future noise-robust approaches. It allows for a range of realistic noisy label sets with varying noise shares, and as a result levels of difficulty, while providing a high-quality clean test set. In addition, \benchmark~ represents a generally harder, but much less ambiguous task.

% cosine doesn't work because we are not using it right - Weak reduced to MV, with a lot of random labels, which COSINE first takes only the subset which is covered.

% indicates that the Rotten Tomatoes task is a relatively easy task, since the discrepancy between the baseline and Oracle subset results is quite small for almost all noise types. 

% Other points:

% 1. Noise shares low, even LLM, excluding Weak with very high noise (almost random labels). Crowd labels around 10\% noise, unlike for NER. For this problem the relationship between different noise sources and their levels is different. 

% 2. All oracle subsets are very close to Clean baseline, meaning much fewer samples are needed to achieve .89 or close to it

% 3. would also mention that LLM noise share is 12 (we can also maybe  add that we got the same number on the test set), which is very close to 89 and looks like fine-tuning doesn't help much. %Easy (few clean samples,...) to get to 87 (even zero-shot LLM does it), but almost impossible to get over 90 (the task is not hard, but probably many ambiguous samples which are impossible to get right). 

% 4. Takeaway: This ablation showcases that realistic noise can have varying degrees of difficulty, depending on the task???

% 5. 'Clean' set is in fact expert (no relabelling rounds like in conll). Reason why Crowd++ upper bound is higher than clean.

% maybe try to frame this setup as a "bad" benchmark for evaluating noise robustness. benefits of NoiseBench for NER: range of noise shares, harder task, high quality clean data available...











==> figures/memorization_plots.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[!htb]{0.3\textwidth}
        \centering
    	\includegraphics[width=\linewidth]{figures/plot100_real_noisy_original.png}
    	\caption{\noiseexpert~noise - 5.9\%}
    	\label{fig:real_original}
    \end{subfigure}
    \begin{subfigure}[!htb]{0.3\textwidth}
        \centering
    	\includegraphics[width=\linewidth]{figures/plot100_real_noisy_mv_oracle.png}
    	\caption{\noisecrowdbest~noise - 15\% }
    	\label{fig:real_mv}
     \end{subfigure}
     \begin{subfigure}[!htb]{0.3\textwidth}
        \centering
		\includegraphics[width=\linewidth]{figures/plot100_real_noisy_bond.png}
    	\caption{\noisedistant~noise - 39\%}
    	\label{fig:real_bond}
     \end{subfigure}
    \begin{subfigure}[!htb]{0.3\textwidth}
        \centering
    	\includegraphics[width=\linewidth]{figures/plot100_simulated_noisy_original.png}
    	\caption{Simulated \noiseexpert~noise - 5.5\%}
    	\label{fig:simulated_original}
    \end{subfigure}
    \begin{subfigure}[!htb]{0.3\textwidth}
        \centering
    	\includegraphics[width=\linewidth]{figures/plot100_simulated_noisy_mv_oracle.png}
    	\caption{Simulated \noisecrowdbest~noise  - 18\%}
    	\label{fig:simulated_mv}
     \end{subfigure}
    \begin{subfigure}[!htb]{0.3\textwidth}
        \centering
    	\includegraphics[width=\linewidth]{figures/plot100_simulated_noisy_bond.png}
    	\caption{Simulated \noisedistant~noise 31\%}
    	\label{fig:simulated_bond}
     \end{subfigure}
\caption{Comparison of the training set F1 score during fine-tuning when the model is trained with a realistic noisy label set versus a corresponding simulated noisy label set. The graphs show both the F1 score on the noisy training labels and on the clean training labels, for 3 different noise types.}
\label{fig:memorization_figure}
\end{figure*}

==> figures/memorization_plots_pyplot_grid.tex <==
\begin{table*}
\centering
\begin{tabular}{@{}ccc@{}}
 \hspace{0.14\textwidth}\noiseexpert & \hspace{0.18\textwidth}\noisecrowdbest & \hspace{0.05\textwidth}\noisedistant \\ 
\multicolumn{3}{c}{
 \includegraphics[width=\linewidth]{figures/memorization_grid.png} }
 \\  
\end{tabular}
\caption{Experiment 2 - Comparison of the training set F1 score during fine-tuning when the model is trained with a realistic noisy label set versus a corresponding simulated noisy label set. The graphs show both the F1 score on the noisy training labels and on the clean training labels, for 3 different noise types.}
\label{fig:memorization_figure}
\end{table*} 


==> figures/seen_vs_unseen_only_real.tex <==
\begin{figure}[!htb]
\centering
 \includegraphics[width=0.49\textwidth]{figures/seen_unseen_plot.png} 
\caption{Real noise: Comparison of F1 scores on different subsets of entities in the test set: all, seen (clean), seen (noisy) and unseen. A similar graph for simulated noise can be found in Appendix \ref{appendix:seen_vs_unseen}.}
\label{fig:seen_vs_unseen_real_only}
\vspace{-2mm}
\end{figure} 

==> figures/seen_vs_unseen_only_simulated.tex <==
\begin{figure}[!htb]
\centering
 \includegraphics[width=\linewidth]{figures/seen_unseen_plot_simulated.png} 
\caption{Simulated class-dependent noise: Comparison of F1 scores on different subsets of entities in the test set: all, seen (clean), seen (noisy) and unseen.}
\label{fig:seen_vs_unseen_simulated_only}
\vspace{-2mm}
\end{figure} 

==> tables/Exp1_real_noise_extended_scores.tex <==
\begin{table*}[]
\setlength{\tabcolsep}{4pt}
\centering
\small
\begin{tabular}{@{}lrrrrrrrr@{}} 
\toprule 
 & \multicolumn{4}{c}{\textit{F1\scriptsize{entity}}} & \multicolumn{4}{c}{\textit{\#Errors}}\\ 
  \cmidrule(lr){2-5} \cmidrule(lr){6-9}  

 & \textit{all} & \textit{seen (clean)} & \textit{seen (noisy)} & \textit{unseen} & \textit{Missing(FN)} & \textit{Boundary(FP)} & \textit{Type} & \textit{Partial match} \\ 
 \midrule
\noiseclean & 93.99 \scriptsize{±0.04} & 95.92 \scriptsize{±0.28} & - & 92.74 \scriptsize{±0.24} & 193.7 \scriptsize{±5.8} & 243.0 \scriptsize{±7.3} & 127.3 \scriptsize{±4.0} & 133.7 \scriptsize{±1.7} \\ 
\noiseexpert & 89.84 \scriptsize{±0.19} & 90.09 \scriptsize{±0.28} & 42.61 \scriptsize{±1.12} & 90.34 \scriptsize{±0.15} & 211.3 \scriptsize{±14.4} & 226.7 \scriptsize{± 3.4} & 363.7 \scriptsize{± 5.8} & 129.7 \scriptsize{± 4.8}\\ 
\noisecrowdbest & 86.71 \scriptsize{±0.29} & 87.22 \scriptsize{±0.54} & 69.13 \scriptsize{±0.77} & 87.18 \scriptsize{±0.16} & 428.7 \scriptsize{± 8.5} & 288.0 \scriptsize{± 1.4} & 393.0 \scriptsize{±12.6} & 176.7 \scriptsize{± 3.7}\\ 
\noisecrowd & 70.52 \scriptsize{±0.62} & 80.62 \scriptsize{±0.54} & 50.79 \scriptsize{±0.60} & 66.80 \scriptsize{±0.70} & 1510.3 \scriptsize{±61.2} & 431.0 \scriptsize{±44.6} & 558.0 \scriptsize{±28.9} & 290.3 \scriptsize{±46.5}\\ 
\noisedistant & 70.75 \scriptsize{±0.13} & 83.49 \scriptsize{±0.29} & 39.71 \scriptsize{±2.66} & 68.28 \scriptsize{±0.31} & 1803.0 \scriptsize{±18.8} & 488.7 \scriptsize{±16.4} & 336.7 \scriptsize{± 8.7} & 298.0 \scriptsize{± 9.6}\\ 
\noiseweak & 65.87 \scriptsize{±0.36} & 81.92 \scriptsize{±0.28} & 23.77 \scriptsize{±0.28} & 62.52 \scriptsize{±0.46} & 643.3 \scriptsize{± 7.8} & 899.0 \scriptsize{±18.4} & 1226.3 \scriptsize{±22.5} & 291.7 \scriptsize{±11.3}\\ 
\noisellm & 62.60 \scriptsize{±0.39} & 68.76 \scriptsize{±0.22} & 28.79 \scriptsize{±0.60} & 63.48 \scriptsize{±0.49} & 825.7 \scriptsize{±17.8} & 1269.0 \scriptsize{±34.8} & 1177.0 \scriptsize{±10.2} & 196.7 \scriptsize{±11.5}\\ 
\bottomrule
 \end{tabular}
 \caption{\label{conll_baselines_real_simulated} F1 scores on the \noiseclean~Test split of the baseline FLERT approach, fine-tuned on different noisy variants of the training set. The scores are averages of 3 runs. The column Difference refers to difference in F1 score on the test split when training on a dataset with simulated noise vs with real noise.
} 
 \end{table*}

==> tables/Exp1_seen_unseen_scores.tex <==
\begin{table*}[]
\setlength{\tabcolsep}{4pt}
\centering
\small
\begin{tabular}{@{}lrrrrrrrr@{}} 
\toprule 
 & \multicolumn{4}{c}{\textit{Real noise}} & \multicolumn{4}{c}{Simulated noise}\\ 
  \cmidrule(lr){2-5} \cmidrule(lr){6-9}  

 & \textit{all} & \textit{seen (clean)} & \textit{seen (noisy)} & \textit{unseen} & \textit{all} & \textit{seen (clean)} & \textit{seen (noisy)} & \textit{unseen} \\ 
 \midrule
\noiseclean & 93.99 \scriptsize{±0.04} & 95.92 \scriptsize{±0.28} & - & 92.74 & - & - & - \\ 
\noiseexpert & 89.84 \scriptsize{±0.19} & 90.09 \scriptsize{±0.28} & 42.61 \scriptsize{±1.12} & 90.34 \scriptsize{±0.15} & 93.74 \scriptsize{±0.21} & 95.58 \scriptsize{±0.34} & 96.30 \scriptsize{±2.62} & 92.51 \scriptsize{±0.21}\\ 
\noisecrowdbest & 86.71 \scriptsize{±0.29} & 87.22 \scriptsize{±0.54} & 69.13 \scriptsize{±0.77} & 87.18 \scriptsize{±0.16} &  88.92 \scriptsize{±0.35} & 94.16 \scriptsize{±0.50} & 87.30 \scriptsize{±2.77} & 85.52 \scriptsize{±0.76}\\ 
\noisecrowd & 70.52 \scriptsize{±0.62} & 80.62 \scriptsize{±0.54} & 50.79 \scriptsize{±0.60} & 66.80 \scriptsize{±0.70} & 72.35 \scriptsize{±1.03} & 77.51 \scriptsize{±1.67} & 51.67 \scriptsize{±1.48} & 71.80 \scriptsize{±0.94} \\ 
\noisedistant & 70.75 \scriptsize{±0.13} & 83.49 \scriptsize{±0.29} & 39.71 \scriptsize{±2.66} & 68.28 \scriptsize{±0.31} & 74.45 \scriptsize{±0.41} & 85.14 \scriptsize{±0.47} & 38.25 \scriptsize{±1.72} & 72.89 \scriptsize{±0.35}\\ 
\noiseweak & 65.87 \scriptsize{±0.36} & 81.92 \scriptsize{±0.28} & 23.77 \scriptsize{±0.28} & 62.52 \scriptsize{±0.46} & 63.05 \scriptsize{±0.77} & 68.94 \scriptsize{±0.38} & 44.24 \scriptsize{±1.75} & 61.25 \scriptsize{±1.19}\\ 
\noisellm & 62.60 \scriptsize{±0.39} & 68.76 \scriptsize{±0.22} & 28.79 \scriptsize{±0.60} & 63.48 \scriptsize{±0.49} & 68.63 \scriptsize{±1.29} & 71.58 \scriptsize{±2.53} & 37.92 \scriptsize{±0.22} & 69.88 \scriptsize{±0.95}\\ 
\bottomrule
 \end{tabular}
 \caption{\label{conll_baselines_real_simulated} F1 scores on the \noiseclean~Test split of the baseline FLERT approach, fine-tuned on different noisy variants of the training set. The scores are averages of 3 runs. The column Difference refers to difference in F1 score on the test split when training on a dataset with simulated noise vs with real noise.
} 
 \end{table*}

==> tables/Exp1_simulated_noise_extended_scores.tex <==
\begin{table*}[]
\setlength{\tabcolsep}{4pt}
\centering
\small
\begin{tabular}{@{}lrrrrrrrr@{}} 
\toprule 
 & \multicolumn{4}{c}{\textit{F1\scriptsize{entity}}} & \multicolumn{4}{c}{\textit{\#Errors}}\\ 
  \cmidrule(lr){2-5} \cmidrule(lr){6-9}  

 & \textit{all} & \textit{seen (clean)} & \textit{seen (noisy)} & \textit{unseen} & \textit{Missing(FN)} & \textit{Boundary(FP)} & \textit{Type} & \textit{Partial match} \\ 
 \midrule
\noiseexpert & 93.74 \scriptsize{±0.21} & 95.58 \scriptsize{±0.34} & 96.30 \scriptsize{±2.62} & 92.51 \scriptsize{±0.21} & 212.3 \scriptsize{±13.8} & 229.3 \scriptsize{±12.4} & 138.3 \scriptsize{±1.7} & 133.0 \scriptsize{±7.0}\\ 
\noisecrowdbest & 88.92 \scriptsize{±0.35} & 94.16 \scriptsize{±0.50} & 87.30 \scriptsize{±2.77} & 85.52 \scriptsize{±0.76} & 577.0 \scriptsize{±27.3} & 483.0 \scriptsize{±27.3} & 99.0 \scriptsize{±7.3} & 418.3 \scriptsize{±28.2}\\ 
\noisecrowd & 72.35 \scriptsize{±1.03} & 77.51 \scriptsize{±1.67} & 51.67 \scriptsize{±1.48} & 71.80 \scriptsize{±0.94} & 1839.0 \scriptsize{±29.5} & 532.0 \scriptsize{±17.9} & 216.7 \scriptsize{±28.5} & 430.7 \scriptsize{±12.8}\\ 
\noisedistant & 74.45 \scriptsize{±0.41} & 85.14 \scriptsize{±0.47} & 38.25 \scriptsize{±1.72} & 72.89 \scriptsize{±0.35} & 1745.3 \scriptsize{±21.7} & 806.3 \scriptsize{±36.0} & 67.0 \scriptsize{±9.9} & 751.3 \scriptsize{±23.6}\\ 
\noiseweak & 63.05 \scriptsize{±0.77} & 68.94 \scriptsize{±0.38} & 44.24 \scriptsize{±1.75} & 61.25 \scriptsize{±1.19} & 882.0 \scriptsize{±54.3} & 860.3 \scriptsize{±63.4} & 1240.0 \scriptsize{±24.9} & 530.0 \scriptsize{±22.0}\\ 
\noisellm & 68.63 \scriptsize{±1.29} & 71.58 \scriptsize{±2.53} & 37.92 \scriptsize{±0.22} & 69.88 \scriptsize{±0.95} & 1298.0 \scriptsize{±52.2} & 783.0 \scriptsize{±39.0} & 674.3 \scriptsize{±63.4} & 467.7 \scriptsize{±63.4}\\ 
\bottomrule
 \end{tabular}
 \caption{\label{conll_baselines_real_simulated} (Simulated noise) F1 scores on the \noiseclean~Test split of the baseline FLERT approach, fine-tuned on different noisy variants of the training set. The scores are averages of 3 runs. The column Difference refers to difference in F1 score on the test split when training on a dataset with simulated noise vs with real noise.
} 
 \end{table*}

==> tables/Exp1_test_errors.tex <==
\begin{table*}[]
\setlength{\tabcolsep}{3pt}
\centering
\small
\begin{tabular}{@{}lcccccccc@{}} 
\toprule 
 & \multicolumn{4}{c}{Real noise} & \multicolumn{4}{c}{Simulated noise}\\ 
  \cmidrule(lr){2-5} \cmidrule(lr){6-9}  

 & \textit{\#Missing(FN)} & \textit{\#Mention(FP)} & \textit{\#Type} & \textit{\#Partial} & \textit{\#Missing(FN)} & \textit{\#Mention(FP)} & \textit{\#Type} & \textit{\#Partial} \\ 
 \midrule
\noiseexpert & 211.3 \scriptsize{±14.4} & 226.7 \scriptsize{± 3.4} & 363.7 \scriptsize{± 5.8} & 129.7 \scriptsize{± 4.8} & 212.3 \scriptsize{±13.8} & 229.3 \scriptsize{±12.4} & 138.3 \scriptsize{±1.7} & 133.0 \scriptsize{±7.0}\\ 
\noisecrowdbest & 428.7 \scriptsize{± 8.5} & 288.0 \scriptsize{± 1.4} & 393.0 \scriptsize{±12.6} & 176.7 \scriptsize{± 3.7} & 577.0 \scriptsize{±27.3} & 483.0 \scriptsize{±27.3} & 99.0 \scriptsize{±7.3} & 418.3 \scriptsize{±28.2}\\ 
\noisecrowd & 1510.3 \scriptsize{±61.2} & 431.0 \scriptsize{±44.6} & 558.0 \scriptsize{±28.9} & 290.3 \scriptsize{±46.5} & 1839.0 \scriptsize{±29.5} & 532.0 \scriptsize{±17.9} & 216.7 \scriptsize{±28.5} & 430.7 \scriptsize{±12.8}\\ 
\noisedistant & 1803.0 \scriptsize{±18.8} & 488.7 \scriptsize{±16.4} & 336.7 \scriptsize{± 8.7} & 298.0 \scriptsize{± 9.6} & 1745.3 \scriptsize{±21.7} & 806.3 \scriptsize{±36.0} & 67.0 \scriptsize{±9.9} & 751.3 \scriptsize{±23.6}\\ 
\noiseweak & 643.3 \scriptsize{± 7.8} & 899.0 \scriptsize{±18.4} & 1226.3 \scriptsize{±22.5} & 291.7 \scriptsize{±11.3} & 882.0 \scriptsize{±54.3} & 860.3 \scriptsize{±63.4} & 1240.0 \scriptsize{±24.9} & 530.0 \scriptsize{±22.0}\\ 
\noisellm & 825.7 \scriptsize{±17.8} & 1269.0 \scriptsize{±34.8} & 1177.0 \scriptsize{±10.2} & 196.7 \scriptsize{±11.5}  & 1298.0 \scriptsize{±52.2} & 783.0 \scriptsize{±39.0} & 674.3 \scriptsize{±63.4} & 467.7 \scriptsize{±63.4}\\ 
\bottomrule
 \end{tabular}
 \caption{\label{conll_baselines_real_vs_simulated_errors} 
} 
 \end{table*}

==> tables/clean_dataset_stats.tex <==
\begin{table}[]
\small
%\setlength{\tabcolsep}{4pt}
\centering
\begin{tabular}{@{}lrrrr@{}}
\toprule
 & \textit{\#Documents} & \textit{\#Sentences} & \textit{\#Entities} & \textit{\#Tokens} \\ \midrule
Train & 400 & 5,885 & 9,685 & 79,720 \\
Test & 231 & 3,427 & 5,725 & 46,504 \\ \bottomrule
\end{tabular}
\caption{\label{clean_dataset_stats} Statistics of the Clean (noise-free) splits}
\vspace{-2mm}
\end{table}


==> tables/conll_confident_learning_acc.tex <==
\begin{table*}[]
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
 & \multicolumn{2}{c}{\textit{before sample selection}} & \multicolumn{2}{c}{\textit{after sample selection}} \\
 & noise share & number of clean sentences & noise share & number of clean sentences \\ \midrule
\noiseclean &  0 & 5215 & 0 & 5061\\
\noiseexpert & 0.0769 & 4814 & 0.0674 & 4722 \\
\noisecrowdbest & 0.2104 & 4118 & 0.1912 & 4019 \\
\noisecrowd & 0.4460 & 2889 & 0.4277 & 2850 \\
\noisedistant &  0.4125 & 3064 & 0.4035 & 3020 \\
\noiseweak & 0.4961 & 2628 & 0.4452 & 2578  \\
\noisellm & 0.6086 & 2041 & 0.5287 & 1936 \\
Average & 0.3215 & 3538.43 & 0.2948 & 3455.14 \\ \bottomrule
\end{tabular}
\caption{\label{Experiment3_CL_accuracy}  }
\end{table*}

==> tables/conll_noise_shares.tex <==
\begin{table*}[]
\centering
\begin{tabular}{c c c }
\toprule
CoNLL-03 label set&F1&\% correct sentences\\ \midrule
\noiseclean   & 100  & 100 \\
\noiseexpert~\citep{tjong-kim-sang-de-meulder-2003-introduction} & 94.5 & 92.6 \\
\noisecrowdbest~\citep{rodrigues2014sequence} & 84.7 & 79.4  \\
\noisecrowd~ & 63.4 & 55.3 \\
\noisedistant~\citep{liang2020bond} & 68.7 & 59.7 \\
\noiseweak~\citep{zhang2021wrench} & 59.6 & 49.6  \\
\noisellm~\citep{golde2023fabricator}& 54.4 & 38.2\\ 
\bottomrule
\end{tabular}
\caption{\label{conll_noise_shares_table} Overview of }
\end{table*}

==> tables/conll_noise_shares_extended.tex <==
\begin{table*}[]
\centering
\begin{tabular}{@{}m{4.8cm} r r r r r r r}
% & \multicolumn{5}{c}{\textit{realistic}} & \multicolumn{5}{c}{\textit{simulated}} \\
 % &  & & \multicolumn{3}{c}{entity-level} & %& token-level F1 & F1 & Prec. & Rec. & No. entities 
 \\
 \toprule
 & \textit{Acc.}\scriptsize{sentence} & \textit{F1}\scriptsize{token}& \textit{F1} & \textit{Prec.} & \textit{Rec.} & \textit{\#Entities} & \textit{Noise level} %& token-level F1 & F1 & Prec. & Rec. & No. entities 
 \\ \midrule
\noiseclean~{\small\citep{ruecker2023clean}} & 100 & 100 & 100 & 100 & 100 & 9,685 & 0 \\ % &  &  &  &  &  
\noiseexpert~{\small\citep{tjong-kim-sang-de-meulder-2003-introduction}} & 92.6 & 99.0 & 94.5 & 94.7 & 94.3 & 9,644 & 5.5 %& 99 & 94.5 & 94.7 & 94.3 & 9644 
\\
\noisecrowdbest~{\small\citep{rodrigues2014sequence}} & 79.4 & 96.8 & 84.7 & 90.1 & 80.0 & 8,607 & 15.3 %& 96.8 & 84.7 & 90.1 & 80 & 8607 
\\
\noisecrowd~{\small\citep{rodrigues2014sequence}} & 55.3 & 92.4 & 63.4 & 74.5 & 55.3 & 7,188 & 36.6 %& 92.4 & 63.4 & 74.5 & 55.3 & 7188 
\\
\noisedistant~{\small\citep{liang2020bond}} & 59.7 & 92.9 & 68.7 & 79.8 & 60.4 & 7,329 & 31.3 %& 92.9 & 68.7 & 79.8 & 60.4 & 7329  
\\
\noiseweak~{\small\citep{zhang2021wrench}} & 49.6 & 92.0 & 59.6 & 56.9 & 62.6 & 10,640 & 40.4  %& 92 & 59.6 & 56.9 & 62.6 & 10640 
\\
\noisellm~{\small\citep{golde2023fabricator}} & 38.2 & 87.4 & 54.4 & 50.5 & 59.1 & 11,349 & 44.6 %& 87.4 & 54.4 & 50.5 & 59.1 & 11349 
\\
\bottomrule
\end{tabular}
\caption{\label{conll_noise_shares_table} Overview of the realistic noisy label sets for CoNLL. The table shows the sentence-level accuracy (\textit{Acc.}), micro-averaged token-level F1 score, as well as micro-averaged entity-level F1, precision (\textit{Prec.}) and recall (\textit{Rec.}).} 

\end{table*}


==> tables/noisebench_overview.tex <==
\begin{table*}[]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}m{5.1cm} r r r r r r r r r r }
% & \multicolumn{5}{c}{\textit{realistic}} & \multicolumn{5}{c}{\textit{simulated}} \\
 % &  & & \multicolumn{3}{c}{entity-level} & %& token-level F1 & F1 & Prec. & Rec. & No. entities 
 \\
 \toprule
 & \textit{Acc.}\scriptsize{sent.}& \textit{F1}\scriptsize{token}& \textit{F1} & \textit{Prec.} & \textit{Rec.} & \textit{\#Entities} & \textit{\#Doc.} & \textit{\#Sent.}  & \textit{\%Noise} %& token-level F1 & F1 & Prec. & Rec. & No. entities 
 \\ \midrule
\textit{Training splits} & & & & & & & & & \\
\noiseclean~{\small\citep{ruecker2023clean}} & 100 & 100 & 100 & 100 & 100 & 9,685 & 400 & 5,885 & 0 \\ % &  &  &  &  &  
\noiseexpert~{\small\citep{tjong-kim-sang-de-meulder-2003-introduction}} & 92.6 & 99.0 & 94.5 & 94.7 & 94.3 & 9,644 & 400 & 5,885 &  5.5 %& 99 & 94.5 & 94.7 & 94.3 & 9644 
\\
\noisecrowdbest~{\small\citep{rodrigues2014sequence}} & 79.4 & 96.8 & 84.7 & 90.1 & 80.0 & 8,607 & 400 & 5,885 & 15.3 %& 96.8 & 84.7 & 90.1 & 80 & 8607 
\\
\noisecrowd~{\small\citep{rodrigues2014sequence}} & 55.3 & 92.4 & 63.4 & 74.5 & 55.3 & 7,188 & 400 & 5,885 &  36.6 %& 92.4 & 63.4 & 74.5 & 55.3 & 7188 
\\
\noisedistant~{\small\citep{liang2020bond}} & 59.7 & 92.9 & 68.7 & 79.8 & 60.4 & 7,329 & 400 & 5,885 & 31.3 %& 92.9 & 68.7 & 79.8 & 60.4 & 7329  
\\
\noiseweak~{\small\citep{zhang2021wrench}} & 49.6 & 92.0 & 59.6 & 56.9 & 62.6 & 10,640 & 400 & 5,885 & 40.4  %& 92 & 59.6 & 56.9 & 62.6 & 10640 
\\
\noisellm~{\small\citep{golde2023fabricator}} & 38.2 & 87.4 & 54.4 & 50.5 & 59.1 & 11,349 & 400 & 5,885 & 44.6 %& 87.4 & 54.4 & 50.5 & 59.1 & 11349 
\\
\midrule 
\textit{Test split} & & & & & & & & &  \\
\noiseclean~Test~{\small\citep{ruecker2023clean}} & 100 & 100 & 100 & 100 & 100 & 5,725 & 231 & 3,427 &  0 \\
\bottomrule
\end{tabular}
\caption{\label{conll_noise_shares_table} Overview of the training and test splits in \benchmark. The table shows the sentence-level accuracy (\textit{Acc.}\scriptsize{sent.}\normalsize), micro-averaged token-level F1 score (\textit{F1}\scriptsize token\normalsize), micro-averaged entity-level F1 (\textit{F1}), precision (\textit{Prec.}), recall (\textit{Rec.}); as well as number of entities (\textit{\#Entities}), documents (\textit{\#Doc.}), sentences (\textit{\#Sent.}) and noise level.} 
\vspace{-2mm}
\end{table*}


==> tables/noisebench_overview_extended.tex <==
\begin{table*}[]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lrrrrrrrrrrr@{}}
\toprule
 & &  & \multicolumn{3}{c}{\textit{Entity-level}} & \multicolumn{2}{c}{\textit{\#Entities}} &\multicolumn{4}{c}{\textit{\#Errors}} \\
 \cmidrule(lr){4-6} \cmidrule(lr){7-8}   \cmidrule(lr){9-12}  
 \textit{Noisy train split} & \textit{\%Noise} & \textit{F1}\scriptsize{token} & \textit{F1} & \textit{Prec.} & \textit{Rec.} & \textit{Total} & \textit{Correct} & \textit{Missing (FN)} & \textit{Mention (FP)} & \textit{Type} & \textit{Partial} \\ 
\midrule %\multicolumn{3}{@{}l}{\textit{Noisy training splits}}\ &  &  &  &  &  &  &  &  &  \\
% \noiseclean & 0 & 100 & 100 & 100 & 100 & 9,685 & 9,685 & 0 & 0 & 0 & 0 \\
\noiseexpert & 5.5 & 99.0 & 94.5 & 94.7 & 94.3 & 9,644 & 9,129 & 133 & 92 & \textbf{423} & 76 \\
\noisecrowdbest & 15.3 & 96.8 & 84.7 & 90.1 & 80.0 & 8,607 & 7,751 & \textbf{1,574} & 496 & 360 & 312 \\
\noisecrowd & 36.6 & 92.4 & 63.4 & 74.5 & 55.3 & 7,188 & 5,352 & \textbf{3,562} & 1,065 & 771 & 574 \\
\noisedistant & 31.3 & 92.9 & 68.7 & 79.8 & 60.4 & 7,329 & 5,846 & \textbf{3,284} & 928 & 555 & 476 \\
\noiseweak & 40.4 & 92.0 & 59.6 & 56.9 & 62.6 & 10,640 & 6,058 & 1,614 & \textbf{2,569} & \textbf{2,013} & 652 \\
\noisellm & 44.6 & 87.4 & 54.4 & 50.5 & 59.1 & 11,349 & 5,726 & 1,903 & \textbf{3,567} & 2,056 & 270 \\
% \midrule 
% \textit{Test split} &  &  &  &  &  &  &  &  &  &  &  \\
% \noiseclean~Test & 0 & 100 & 100 & 100 & 100 & 5,725 & 5,725 & 0 & 0 & 0 & 0 \\
\bottomrule
\end{tabular}
\caption{\label{conll_noise_shares_table} Overview of the noisy training splits in \benchmark. The table shows the noise level, the micro-averaged token-level F1 score (\textit{F1}\begin{scriptsize} token \end{scriptsize}), micro-averaged entity-level F1 (\textit{F1}), precision (\textit{Prec.}), recall (\textit{Rec.}); as well as the number of entities (\textit{\#Entities}) and number of correct entities (\textit{\#Correct}). It also shows the number of incorrect entities for each type of error: missing boundaries (\textit{Missing(FN)}), incorrectly labeled mentions with a wrong boundary (\textit{Mention(FN)}) and wrong type (\textit{Type}), as well as the number of partial matches (\textit{Partial}).} 
\vspace{-2mm}
\end{table*}

==> tables/noisebench_overview_merged.tex <==
\begin{table*}[]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrrrrrrrrrr@{}}
\toprule
 &  & & & & & \multicolumn{2}{c}{\textit{\#Entities}} &\multicolumn{4}{c}{\textit{\#Errors}} \\
 \cmidrule(lr){7-8}   \cmidrule(lr){9-12}  
& \textit{\%Noise} & \textit{F1}\scriptsize{token} & \textit{F1} & \textit{Prec.} & \textit{Rec.} & \textit{Total} & \textit{Correct} & \textit{Missing(FN)} & \textit{Boundary(FP)} & \textit{Type} & \textit{Partial} & \textit{\#Doc.} & \textit{\#Sent.}  \\ \midrule \multicolumn{4}{@{}l}{\textit{Noisy training splits}}\  &  &  &  &  &  &  &  &  && \\
\noiseclean & 0 & 100 & 100 & 100 & 100 & 9,685 & 9,685 & 0 & 0 & 0 & 0 & 400 & 5,885 \\
\noiseexpert & 5.5 & 99.0 & 94.5 & 94.7 & 94.3 & 9,644 & 9,129 & 133 & 92 & 423 & 76 & 400 & 5,885\\
\noisecrowdbest & 15.3 & 96.8 & 84.7 & 90.1 & 80.0 & 8,607 & 7,751 & 1,574 & 496 & 360 & 312 & 400 & 5,885\\
\noisecrowd & 36.6 & 92.4 & 63.4 & 74.5 & 55.3 & 7,188 & 5,352 & 3,562 & 1,065 & 771 & 574 & 400 & 5,885\\
\noisedistant & 31.3 & 92.9 & 68.7 & 79.8 & 60.4 & 7,329 & 5,846 & 3,284 & 928 & 555 & 476 & 400 & 5,885\\
\noiseweak & 40.4 & 92.0 & 59.6 & 56.9 & 62.6 & 10,640 & 6,058 & 1,614 & 2,569 & 2,013 & 652 & 400 & 5,885\\
\noisellm & 44.6 & 87.4 & 54.4 & 50.5 & 59.1 & 11,349 & 5,726 & 1,903 & 3,567 & 2,056 & 270 & 400 & 5,885\\
\midrule 
\textit{Test split} &  &  &  &  &  &  &  &  &  &  & & & \\
\noiseclean~Test & 0 & 100 & 100 & 100 & 100 & 5,725 & 5,725 & 0 & 0 & 0 & 0& 231 & 3,427 \\
\bottomrule
\end{tabular}
\caption{\label{conll_noise_shares_table} Overview of the noisy training splits in \benchmark. The table shows the noise level, the micro-averaged token-level F1 score (\textit{F1}\begin{scriptsize} token \end{scriptsize}), micro-averaged entity-level F1 (\textit{F1}), precision (\textit{Prec.}), recall (\textit{Rec.}); as well as the number of entities (\textit{\#Entities}) and number of correct entities (\textit{\#Correct}). It also shows the number of incorrect entities for each type of error: missing boundaries (\textit{Missing(FN)}), incorrectly labeled mentions with a wrong boundary (\textit{Boundary(FN)}) and wrong type (\textit{Type}), as well as the number of partial matches (\textit{Partial}).} 
\vspace{-2mm}
\end{table*}

==> tables/noisebench_overview_shares_short.tex <==
\begin{table}[]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
 & & &  & &\multicolumn{4}{c}{\textit{\%Errors}} \\
  \cmidrule(lr){5-6}   \cmidrule(lr){7-9}  
 \textit{Variant} & \textit{\%} & \textit{F1}\scriptsize{tok.} & \textit{F1\scriptsize{ent.}} & \textit{Total} & \textit{FN} & \textit{FP} & \textit{Type} & \textit{Partial} \\ 
\midrule %\multicolumn{3}{@{}l}{\textit{Noisy training splits}}\ &  &  &  &  &  &  &  &  &  \\
% \noiseclean & 0 & 100 & 100 & 100 & 100 & 9,685 & 9,685 & 0 & 0 & 0 & 0 \\
\noiseexpert & 5.5 & 99.0 & 94.5 & 9644  & 10.0 & 2.8 & 74.0 & 13.3 \\
\noisecrowdbest & 15.3 & 96.7 & 84.7 & 8607  & 59.6 & 8.7 & 17.0 & 14.7 \\
\noisecrowd & 36.6 & 92.3 & 63.4 & 7188  & 61.9 & 10.2 & 16.0 & 11.9 \\
\noisedistant & 31.3 & 92.9 & 68.7 & 7329  & 65.4 & 10.5 & 12.9 & 11.1 \\
\noiseweak & 40.4 & 91.9 & 59.6 & 10640  & 17.4 & 34.6 & 36.3 & 11.8 \\
\noisellm &  45.6 & 87.4 & 54.4 & 11349 & 22.5 & 45.4 & 28.3 & 3.7 \\
% \midrule 
% \textit{Test split} &  &  &  &  &  &  &  &  &  &  &  \\
% \noiseclean~Test & 0 & 100 & 100 & 100 & 100 & 5,725 & 5,725 & 0 & 0 & 0 & 0 \\
\bottomrule
\end{tabular}
\caption{\label{conll_noise_shares_table} Overview of the noisy training splits in \benchmark. The table shows the noise level, the micro-averaged token-level F1 score (\textit{F1}\begin{scriptsize} token \end{scriptsize}), micro-averaged entity-level F1 (\textit{F1}), precision (\textit{Prec.}), recall (\textit{Rec.}); as well as the number of entities (\textit{\#Entities}) and number of correct entities (\textit{\#Correct}). It also shows the number of incorrect entities for each type of error: missing mentions (\textit{Missing (FN)}), incorrectly labeled mentions with a wrong boundary (\textit{Non-entity (FN)}) and wrong type (\textit{Type}), as well as the number of partial matches (\textit{Partial}).} 
\vspace{-2mm}
\end{table}

==> tables/noisebench_overview_shortened.tex <==
\begin{table}[]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}l r r r r r r }
% & \multicolumn{5}{c}{\textit{realistic}} & \multicolumn{5}{c}{\textit{simulated}} \\
 % &  & & \multicolumn{3}{c}{entity-level} & %& token-level F1 & F1 & Prec. & Rec. & No. entities 
 \\
 \toprule
 & \textit{F1}\scriptsize{token}& \textit{F1} & \textit{Prec.} & \textit{Rec.} & \textit{\#Entities} & \textit{\%Noise} %& token-level F1 & F1 & Prec. & Rec. & No. entities 
 \\ \midrule
\multicolumn{2}{l}{\textit{Training splits}} & & & & & \\
\noiseclean &  100 & 100 & 100 & 100 & 9,685 &  0 \\ % &  &  &  &  &  
\noiseexpert &  99.0 & 94.5 & 94.7 & 94.3 & 9,644 &  5.5 %& 99 & 94.5 & 94.7 & 94.3 & 9644 
\\
\noisecrowdbest & 96.8 & 84.7 & 90.1 & 80.0 & 8,607 &  15.3 %& 96.8 & 84.7 & 90.1 & 80 & 8607 
\\
\noisecrowd &  92.4 & 63.4 & 74.5 & 55.3 & 7,188 &   36.6 %& 92.4 & 63.4 & 74.5 & 55.3 & 7188 
\\
\noisedistant &  92.9 & 68.7 & 79.8 & 60.4 & 7,329 &  31.3 %& 92.9 & 68.7 & 79.8 & 60.4 & 7329  
\\
\noiseweak &  92.0 & 59.6 & 56.9 & 62.6 & 10,640 & 40.4  %& 92 & 59.6 & 56.9 & 62.6 & 10640 
\\
\noisellm & 87.4 & 54.4 & 50.5 & 59.1 & 11,349 &  44.6 %& 87.4 & 54.4 & 50.5 & 59.1 & 11349 
\\
% \midrule 
% \textit{Test split} & & & & & & & & &  \\
% \noiseclean~Test~{\small\citep{ruecker2023clean}} & 100 & 100 & 100 & 100 & 100 & 5,725 & 231 & 3,427 &  0 \\
\bottomrule
\end{tabular}
\caption{\label{conll_noise_shares_table} Overview of the training and test splits in \benchmark. The table shows the micro-averaged token-level F1 score (\textit{F1}\scriptsize token\normalsize), micro-averaged entity-level F1 (\textit{F1}), precision (\textit{Prec.}), recall (\textit{Rec.}); as well as number of entities (\textit{\#Entities}), documents (\textit{\#Doc.}), sentences (\textit{\#Sent.}) and noise level.} 
\vspace{-2mm}
\end{table}


==> tables/rotten-tomatoes-sentiment/rt_confident_learning_acc.tex <==
\begin{table*}[]
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
 & \multicolumn{2}{c}{\textit{before sample selection}} & \multicolumn{2}{c}{\textit{after sample selection}} \\
 & noise share & number of clean sentences & noise share & number of clean sentences \\ \midrule
\noiseclean & 0 & 4249 & 0 & 3605 \\
\noisecrowdbest & 0.0901 & 3866 & 0.0601 & 3409 \\
\noisecrowd & 0.1099 & 3782 & 0.0665 & 3325 \\
\noiseweak & 0.4450 & 2358 & 0.3621 & 1614 \\
\noisellm &  0.1200 & 3739 & 0.0839 & 3331 \\
Average & 0.1530	& 3598.8 & 0.1145 & 3056.8   \\ \bottomrule
\end{tabular}
\caption{\label{Experiment3_CL_accuracy_rt}  Performance of the confident learning approach for clean sample selection on the \rottentomatoes~dataset. The first two columns show the noise share and total number of clean sentences in the original datasets (\textit{before sample selection}). The second two columns show the noise share and total number of clean sentences of the data subset selected as clean (\textit{after sample selection}). We can see that the noise share of the selected subset is lower than the noise share of the original dataset for every noise level. However, the total number of clean samples decreases as well.}
\end{table*}



==> tables/rotten-tomatoes-sentiment/rt_noise_shares.tex <==
\begin{table}[]
\centering
\begin{tabular}{@{}p{3.3cm} r r @{}}
\toprule
 & \textit{Noise level} & \% \textit{"positive"}\\ \midrule
\makecell[l]{ \noiseclean~\\{\small\citep{pang-lee-2005-seeing}} }     & 0 & 50.05   \\
\makecell[l]{\noisecrowdbest~\\{\small\citep{rodrigues2013learning}}  } & 8.9 & 47.19\\
\makecell[l]{\noisecrowd~\\{\small\citep{rodrigues2013learning}} } & 11.0   & 50.53     \\
\makecell[l]{\noisellm~\\{\small\citep{golde2023fabricator}} } & 12.1 & 49.52 \\
\makecell[l]{\noiseweak~\\{\small\citep{zhang2021wrench}} } & 44.5 & 53.77 \\
\bottomrule
\end{tabular}
\caption{\label{RT_noise_shares_table} Overview of the realistic noisy label sets for \rottentomatoes. }
\end{table}

==> tables/rotten-tomatoes-sentiment/rt_results.tex <==
\begin{table*}[]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{p{3cm} r r r r r r r r}
\toprule
 & \noiseclean & \noisecrowdbest & \noisecrowd & \noiseweak & \noisellm & Average \tabularnewline \midrule
\%Noise & - & 8.9 & 11.0 & 44.5 & 12.1 & - \tabularnewline \midrule
Baseline & 89.28{\scriptsize±0.07} & 88.79{\scriptsize±0.12} & 88.07{\scriptsize±0.22} & 65.45{\scriptsize±1.02} & 86.43{\scriptsize±0.09} & 83.60 \tabularnewline  \midrule
 \multicolumn{3}{l}{\textit{Upper bounds}} & & & & & & \tabularnewline
Oracle subset & - & 89.42{\scriptsize±0.09} & 89.13{\scriptsize±0.11} & 87.70{\scriptsize±0.32} & 88.45{\scriptsize±0.27} & \textbf{88.68}  \tabularnewline
Oracle stopping & 89.43 {\scriptsize±0.20} & 88.81{\scriptsize±0.07} & 88.42{\scriptsize±0.06} & 70.45{\scriptsize±2.98} & 87.19{\scriptsize±0.16} &  84.86\tabularnewline 
\midrule
 \multicolumn{3}{l}{\textit{Noise-robust learning}} & & & & & &  \tabularnewline
Co-regularization & \textbf{89.76}{\scriptsize±0.15} & \textbf{89.36}{\scriptsize±0.24} & \textbf{88.92}{\scriptsize±0.14} & \textbf{72.21}{\scriptsize±2.00} & \textbf{87.94}{\scriptsize±0.17} & 85.64 \tabularnewline
Confident learning &88.93{\scriptsize±0.16} & 88.59{\scriptsize±0.07} & 88.00{\scriptsize±0.09} & 72.03{\scriptsize±0.48} & 86.94{\scriptsize±0.19} & 84.90 \tabularnewline
COSINE & 88.83{\scriptsize±0.36} & 88.48{\scriptsize±0.44} & 88.62{\scriptsize±0.16} & 61.50{\scriptsize±10.18} & 86.92{\scriptsize±0.08} & 82.87 \tabularnewline 
%\midrule \multicolumn{3}{l}{\textit{zero-shot}} & & & & & & \tabularnewline LLM & 87.82 & & & & & & \tabularnewline
\bottomrule
\end{tabular}
\caption{\label{exp3_rt_results} Performance of noise-robust approaches on the Clean RT-MR test set, when training on \benchmark{} label sets. Results are expressed in terms of Accuracy score. Each score is averaged over 3 runs.}
\end{table*}

==> tables/simulated_noise_overview.tex <==
\begin{table*}[]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lrrrrrrrrrrr@{}}
\toprule
 &  & & & & & \multicolumn{2}{c}{\textit{\#Entities}} &\multicolumn{4}{c}{\textit{\#Errors}} \\
 \cmidrule(lr){7-8}  \cmidrule(lr){9-12}  
& \textit{\%Noise} & \textit{F1}\scriptsize{token} & \textit{F1} & \textit{Prec.} & \textit{Rec.} & \textit{\#Entities} & \textit{\#Correct} & \textit{Missing (FN)} & \textit{Mention (FP)} & \textit{Type} & \textit{Partial} \\ \midrule
\textit{Training splits} &  &  &  &  &  &  &  &  &  &  &  \\
\noiseclean & 0 & 100 & 100 & 100 & 100 & 9,685 & 9,685 & 0 & 0 & 0 & 0 \\
\noiseexpert & 5.9 & 99 & 94.5 & 94.7 & 94.3 & 9,680 & 9,114 & 210 & 205 & 361 & 112 \\
\noisecrowdbest & 17.9 & 96 & 82.1 & 86.8 & 77.8 & 8,686 & 7,537 & 1,854 & 855 & 294 & 530 \\
\noisecrowd & 41.3 & 91.2 & 58.7 & 68.5 & 51.4 & 7,278 & 4,982 & 4,048 & 1,641 & 655 & 912 \\
\noisedistant & 39.2 & 92.2 & 60.8 & 69.7 & 53.9 & 7,496 & 5,224 & 3,961 & 1,772 & 500 & 1,103 \\
\noiseweak & 41.2 & 91.8 & 58.8 & 55.7 & 62.2 & 10,814 & 6,023 & 1,995 & 3,124 & 1,667 & 795 \\
\noisellm & 47.2 & 88.8 & 52.8 & 48.3 & 58.1 & 11,640 & 5,626 & 2,256 & 4,211 & 1,803 & 419 \\
\bottomrule
\end{tabular}
\caption{\label{conll_noise_shares_table_simulated} (Simulated noise) Overview of the training and test splits in \benchmark. The table shows the noise level, the micro-averaged token-level F1 score (\textit{F1}\begin{scriptsize} token\end{scriptsize}), micro-averaged entity-level F1 (\textit{F1}), precision (\textit{Prec.}), recall (\textit{Rec.}); as well as number of entities (\textit{\#Entities}) and number of correct entities (\textit{\#Correct}). It also shows the number of incorrect entities for each type of error: missing boundaries (\textit{Missing(FN)}), incorrectly labeled mentions with a wrong boundary (\textit{Mention(FP)}) and wrong type (\textit{Type}), as well as the number of partial matches (\textit{Partial}). } 
\vspace{-2mm}
\end{table*}

==> tables/simulated_vs_real_noise.tex <==
\begin{table*}[]
\setlength{\tabcolsep}{4pt}
\centering
\small
\begin{tabular}{lccccc}
\toprule
%  &  & \multicolumn{2}{c}{ F1 }\\ \midrule
% \noiseclean &  & \multicolumn{2}{c}{93.99 ± 0.04}\\ \midrule
  &  \multicolumn{2}{c}{ Real noise } & \multicolumn{2}{c}{ Simulated noise } & Difference\\ \midrule
 & \%Noise & F1 & \%Noise & F1 & F1 \\ \midrule
 \noiseclean & 0 & 93.99\scriptsize{±0.04} & - & - & - \\
\noiseexpert & 5.5 & 89.84\scriptsize{±0.19} & 5.9 & 93.74\scriptsize{±0.21} & 3.90 \\
\noisecrowdbest & 15.3 & 86.71\scriptsize{±0.29} & 17.9 & 88.92\scriptsize{±0.35} & 2.21 \\
\noisecrowd & 36.6 & 70.52\scriptsize{±0.62} & 41.3 & 72.35\scriptsize{±1.03} & 1.83\\
\noisedistant & 31.3 & 70.75\scriptsize{±0.13} & 39.2 & 74.45\scriptsize{±0.41} & 3.70 \\
\noiseweak & 40.4 & 65.87\scriptsize{±0.36} & 41.2 & 63.05\scriptsize{±0.77} & -2.82 \\
\noisellm & 44.6 & 62.60\scriptsize{±0.39} & 47.2 & 68.63\scriptsize{±1.29} &6.03 \\ 
Average &  & 74.38\scriptsize{±0.33} & & 76.86\scriptsize{±0.67} & 2.48 \\ \bottomrule
\end{tabular}
\caption{\label{conll_baselines_real_simulated} F1 scores on the \noiseclean~Test split of the baseline FLERT approach, fine-tuned on different noisy variants of the training set. The scores are averages of 3 runs. The column Difference refers to difference in F1 score on the test split when training on a dataset with simulated noise vs with real noise.
} %The scores are averaged over 3 runs. Training on the clean training set has a score of 93.99}%\scriptsize{±0.04}}
\vspace{-2mm}
\end{table*}


==> tables/simulated_vs_real_noise_with_token_noise.tex <==
\begin{table*}[]
\setlength{\tabcolsep}{4pt}
\centering
\small
\begin{tabular}{lccccccc}
\toprule
%  &  & \multicolumn{2}{c}{ F1 }\\ \midrule
% \noiseclean &  & \multicolumn{2}{c}{93.99 ± 0.04}\\ \midrule
  &  \multicolumn{3}{c}{ Real noise } & \multicolumn{3}{c}{ Simulated noise } & Difference\\   \cmidrule(lr){2-4} \cmidrule(lr){5-7}  
 & \%Noise\scriptsize{ token }& \%Noise & F1 & \%Noise\scriptsize{ token }& \%Noise & F1 & F1 \\ \midrule
 \noiseclean & 0 & 0 & 93.99\scriptsize{±0.04} & - & - & - & - \\
\noiseexpert & 1 & 5.5 & 89.84\scriptsize{±0.19} & 1 & 5.9 & 93.74\scriptsize{±0.21} & 3.90 \\
\noisecrowdbest & 3.3 & 15.3 & 86.71\scriptsize{±0.29} & 4 & 17.9 & 88.92\scriptsize{±0.35} & 2.21 \\
\noisecrowd & 7.7 & 36.6 & 70.52\scriptsize{±0.62} & 8.8 & 41.3 & 72.35\scriptsize{±1.03} & 1.83\\
\noisedistant & 7.1 & 31.3 & 70.75\scriptsize{±0.13} & 7.8 & 39.2 & 74.45\scriptsize{±0.41} & 3.70 \\
\noiseweak & 8.1 & 40.4 & 65.87\scriptsize{±0.36} & 8.2 & 41.2 & 63.05\scriptsize{±0.77} & -2.82 \\
\noisellm & 12.6 & 45.6 & 62.60\scriptsize{±0.39} & 11.2 & 47.2 & 68.63\scriptsize{±1.29} &6.03 \\ 
Average & & & 74.38\scriptsize{±0.33} & & & 76.86\scriptsize{±0.67} & 2.48 \\ \bottomrule
\end{tabular}
\caption{\label{conll_baselines_real_simulated} F1 scores on the \noiseclean~Test split of the baseline FLERT approach, fine-tuned on different noisy variants of the training set. The scores are averages of 3 runs. The column Difference refers to difference in F1 score on the test split when training on a dataset with simulated noise vs with real noise.
} %The scores are averaged over 3 runs. Training on the clean training set has a score of 93.99}%\scriptsize{±0.04}}
\vspace{-2mm}
\end{table*}

